Thought Graph: Generating Thought Process for Biological Reasoning

We present the Thought Graph as a novel framework to support complex reasoning and use gene set analysis as an example to uncover semantic relationships between biological processes. Our framework stands out for its ability to provide a deeper understanding of gene sets, significantly surpassing GSEA by 40.28% and LLM baselines by 5.38% based on cosine similarity to human annotations. Our analysis further provides insights into future directions of biological processes naming, and implications for bioinformatics and precision medicine.

==> analysis.tex <==
\ethan{to write} 

\begin{figure}[t]
    \includegraphics[width=\linewidth]{images/violent_pot.pdf}
    \centering
	 \caption{} 
% 	 \vspace{-1.0pc}
    \label{fig:vio}
\end{figure}


\subsection{Evaluating \bptree}
In this section, we evaluate the biological processes in \bptree generated by \system. As shown in Tab. \ref{table:performance}, the ToT-GG (b) are able to generate a graph that consists of biological process that is highly similar to the annotated process, with yield 67.32\% similarity score, and 96.96\% of the generated process are significantly better than any terms in GO, defeating the GSEA. 
% \subsection{Accuracy of Graph Structure Generation} 
% \subsection{Effectiveness of ToT in Identifying Correct Answers}

\subsection{Optimal Layer Analysis} 
\subsection{Role of GProfiler in Enhancing LLM Performance} 
\subsection{Consensus in ToT Voting Mechanism} 
\subsection{Balance of Cost and Accuracy}

==> introduction_origin.tex <==
% We are confronted with increasingly sophisticated issues ranging from climate change to drug discovery, which require us to interact with our cognitive processes to enable complex reasoning in the intricate context that we are facing. Complex reasoning follows Allen Newell's principle of rationality, which means that if an agent knows that one of its actions will lead to one of its goals, the agent will select that action \cite{anderson2013adaptive}. The complication is that multiple actions may be required to achieve a goal, or multiple goals will conflict with the actions they selected. 
% Therefore, knowledge is important to constrain actions and define different goals \cite{newell1982knowledge}. 
We are confronted with complex challenges such as climate change and drug discovery that demand sophisticated reasoning, requiring cognitive processes in system design. 
Allen Newell's principle of rationality in knowledge-based systems posits that individuals and agents choose actions they believe will most effectively achieve their goals~\cite{newell1982knowledge}, based on their situational understanding. 
% This principle underlines that rational actions align with goals through perceived effective means. 
The complication is that decision-making in complex environments becomes nuanced when multiple actions could achieve a goal or when goals themselves conflict. Therefore, external knowledge plays a critical role in guiding action selection and goal definition.
% Large Language Models (LLMs) can successfully mimic human cognitive reasoning that Chain-of-Thoughts (CoT), Tree-of-Thoughts (ToT), and Graph-of-Thoughts (GoT) have been successfully applied in different domains \cite{besta2023graph}. 
% But 
% However, none of the existing Large Language Model (LLM) frameworks aligns with it by integrating goal, action, and knowledge together rather than just forming a sequence of actions \cite{anderson2013adaptive}.
% to realize goals without recalling outside knowledge \cite{anderson2013adaptive}. 
To follow the principle of rationality, especially bringing outside knowledge into the thinking process, we propose the \textbf{Thought Graph} to highlight two important components during the complex reasoning: 1) refining goals by redefining subgoals using external knowledge: we redefine subgoals in each layer of Thought Graph by consulting a voter LLM from the external knowledge to vote for the next steps; 2) recalling external knowledge bases from specific domains to infer edge semantics of Thought Graph to generate semantic relationships (e.g., is-a, part-of) among different thought steps.

Systematic study of human disease requires a comprehensive understanding of the connections between diseases, drugs, phenotypes, genes, and biological processes \cite{chandak2023building}. 
Interpreting biological processes of gene sets that share common biological functions, chromosomal locations, or regulation can uncover collective behaviors of genes in states of health and diseases to enable precision medicine for cancer treatment \cite{doi:10.1073/pnas.0506580102}. 
% Biomedicine is a knowledge-intensive domain with rich knowledge graphs to capture intricate relationships among diverse biological entities \cite{doi:10.1073/pnas.0506580102}. 
However, extracting biological processes from a set of genes poses great challenges in that individual genes tend to have weak signals, and a set of genes with strong signals do not have a unified biological theme, especially different groups studying the same biological system can draw drastically different conclusions \cite{doi:10.1073/pnas.0506580102}. In this paper, we apply Thought Graph as a framework of complex reasoning to derive biological processes from gene sets. Our novel contributions can be summarized as follows:

%Newell \cite{newell1982knowledge} emphasized that if the task is complex enough that additional knowledge from outside of the local context should be recalled at some point during the processing. 

% These problems demand that we leverage complex reasoning in the intricate context that we are facing. %\cite{Knauff2010-ra}. 
% Complex reasoning follows the principle of rationality, 
% The challenge is that multiple actions may be required to achieve a goal, or multiple goals will conflict with the actions they selected.

% Chain-of-Thoughts (CoT), Tree-of-Thoughts (ToT), and Graph-of-Thoughts (GoT) are attempts to imitate human cognitive reasoning that have been successfully applied across different domains \cite{besta2023graph}. But while these frameworks form sequences of actions to realize goals, they do not align with the principle of rationality by also integrating knowledge \cite{anderson2013adaptive}. In accordance with the principle of rationality, with a particular emphasis on bringing outside knowledge into the reasoning process, we propose the \textbf{\system} to highlight two important components during the complex reasoning process: 1) refining goals by redefining subgoals using external knowledge: we redefine subgoals in each layer of \system by consulting a voter LLM agent from the external
% knowledge to vote for the next step; 2) recalling external knowledge bases from specific domains to infer edge semantics of \system to generate semantic relationships (e.g., \textit{is a}, \textit{part of}) across thought steps.

% Large Language Models (LLMs) can successfully mimic human cognitive reasoning that Chain-of-Thoughts (CoT), Tree-of-Thoughts (ToT) and Graph-of-Thoughts (GoT) have been successfully applied in
% different domains \cite{besta2023graph}. 
% But none of them align with the principle of rationality by integrating goal, action, and knowledge together rather than just forming a sequence of actions to realize goals without recalling outside knowledge \cite{anderson2013adaptive}. To follow the principle of rationality, especially bringing outside knowledge into the thinking process, we propose the \textbf{\system} to highlight two important components during the complex reasoning: 1) refining goals by redefining subgoals using external knowledge: we
% redefine subgoals in each layer of \system by consulting a voter LLM agent from the external
% knowledge to vote for the next steps; 2) recalling external knowledge bases from specific domains to infer
% edge semantics of \system to generate semantic relationships (e.g., is-a, part-of) among different thought
% steps.

% Systematic study of human disease requires a comprehensive understanding of the connections
% between diseases, drugs, phenotypes, genes, and biological processes \cite{chandak2023building}.  
% %and other entities, which are crucial for research about phenotyping, drug-disease relationship, drug repurposing, and combination therapies. 
% Interpreting biological processes of gene sets that share common biological functions, chromosomal locations, or regulation can uncover collective behaviors of genes in states of health and diseases to enable precision medicine for cancer treatment \cite{doi:10.1073/pnas.0506580102}. Biomedicine is a knowledge-intensive domain
% with rich knowledge graphs to capture intricate relationships among diverse biological entities \cite{doi:10.1073/pnas.0506580102}. 
% %genes, drugs, diseases, and pathways \cite{doi:10.1073/pnas.0506580102, su2021ibkh, ashburner2000gene}. 
% However, extracting biological processes from a set of genes poses a great challenge, because individual genes tend to have weak signals and sets of of genes with strong signals do not necessarily have a unified biological theme. As a consequence, different groups studying the same biological system can draw drastically different conclusions 
% %showing distressingly litter overlap 
% \cite{doi:10.1073/pnas.0506580102}. In this paper, we apply \system as a framework for
% complex reasoning to derive biological processes from gene sets. Our novel contributions can be
% summarized as follows:
% \vspace{-0.5cm}
\begin{enumerate}
    \item We propose Thought Graph as a complex reasoning framework by incorporating external knowledge during the reasoning process to integrate goal, action, and knowledge together to enable cognitive reasoning according to the principle of rationality.
    \item Thought Graph can generate thought graphs with edge semantics by recalling external knowledge (e.g., Gene Ontology) to build rich semantics among thought steps.
    \item We have successfully applied Thought Graph in biological process generation with significant improvement compared to SOTA methods, surpassing GSEA by 40.28\% and LLM baselines by 5.38\% in cosine similarity score, and identified the optimal steps of complex reasoning by balancing specificity and accuracy.
    % \item We have successfully applied \system in biological process generation with noteworthy improvement compared to SOTA methods, and identified the optimal steps of complex reasoning by balancing specificity and accuracy.
\end{enumerate}
% \vspace{-1.cm}
% \begin{enumerate}
%     \item \system is a complex reasoning framework that uniquely incorporates an external knowledgebase during its reasoning process to integrate goal, action, and knowledge to
% enable cognitive reasoning according to the principle of rationality.
%     \item \system can generate thought graphs with edge semantics by recalling external knowledge (e.g., Gene Ontology) to build rich semantics among thought steps.
%     \item We have successfully applied \system in biological process generation with significant improvement compared to SOTA methods, surpassing GSEA by 42.96\% and LLM baselines by 5.38\%, and identified the optimal steps of reasoning by balancing specificity and accuracy.
%     % \item We have successfully applied \system in biological process generation with noteworthy improvement compared to SOTA methods, and identified the optimal steps of complex reasoning by balancing specificity and accuracy.
% \end{enumerate}

% \ethan{to write} 
% \ethan{didn't propose a new framework; rather, evaluate how ToT performs in this task. --> Explain why this is important. Explainability and interoperability for researchers in Bioinformatics.}
% \ethan{Thought graph does not capture the biological meaning of the graph. We need to think of a better name. }
% \ethan{we're also using ToT slightly different than the original ToT, we use it to generate a coherent graph (explore the most relevant , and ToT use it to generate a path to solution}

% \subsection{Biological Process Term Generation}
% In the field of genomics, it is well-established that sets of genes are differentially expressed to facilitate various biological functions \kyle{cite}. To understand how groups of related genes behave together under different conditions, biologists turn to gene set analysis, which refers to the mapping of sets of genes to the biological processes with which they are associated. To automate this process, researchers have built enrichment analysis tools \ethan{cite}, which use statistical methods to label sets of genes with relevant biological processes by referencing pre-existing gene function databases.
% In the field of genomics, it is well-established that sets of genes are differentially expressed to facilitate various biological functions \kyle{cite}. To understand how groups of related genes behave together under different conditions, earlier studies primarily utilized gene set analysis tools such as gene set enrichment analysis (GSEA)~\cite{doi:10.1073/pnas.0506580102}. More recently, several studies have begun to adopt Large Language Models (LLMs)~\cite{hu2023evaluation} \ethan{cite more}, utilizing the embedded biological knowledge and their reasoning ability. Specifically, Hu et al. explored the application of LLMs for gene set analysis~\cite{hu2023evaluation}, particularly in generating one predominant biological process term and corresponding analysis for each gene set. 

% % large corpus of embedded biological knowledge and recent studies in multi-step in-context reasoning ability.

% % However, the gene function databases used by enrichment tools are incomplete and must be regularly updated as biological literature sheds new light on the relationships between genes and biological functions \kyle{cite}. A natural question is whether a computational tool can be built that performs end-to-end gene set analysis by dynamically reasoning over a large biological knowledgebase to label gene sets without the need for manual literature review and annotation. Large language models (LLMs), because of their large corpus of embedded biological knowledge and multi-step in-context reasoning ability, are strong candidates for this task.

% Expanding on prior research, our study introduces a novel approach for gene set analysis termed ``biological process graph generation,''. This method generates a biological process tree graph, or \textbf{\bptree}, that captures the diverse aspects of gene sets, extending beyond the identification of the most predominant process. 
% \ethan{\textbf{\bptree} suggests a conceptual, thought-like mapping of biological processes, which aligns with the method's approach of creating a graph-based representation of gene ontology. }

% The \bptree approach focuses on both breadth and depth, encompassing a wider array of biological processes (breadth) while also offering options for greater specificity (depth). This dual focus allows for a more comprehensive understanding of the biological processes associated with gene sets. To this end,
% In line with these objectives, we designed \textbf{\system}, a Tree-of-thoughts \cite{yao2023tree} adaption framework for generating a curated tree graph \bptree.
% \ethan{thought graph and thought graph. }

% The \system framework, adapted from the Tree-of-Thoughts (ToT) generation model, aims to create diverse and accurate biological process graphs for gene sets. Drawing inspiration from Gene Ontology \cite{article}, \system structures its output with root-level nodes representing broad biological processes, while leaf-level nodes detail more specific ones. The process begins with the framework's initial expansion in step 1, where an LLM uses the gene set to generate three relevant biological processes. State evaluators then review these and select the two most promising processes. From step 2 to step 5, for each chosen process, the gene set and the process are input back into the LLM to generate a more specific biological process and its relation to the preceding one. This iterative process continues until \system produces a comprehensive tree, where each node signifies a biological process, and edges represent their dependencies. Then, \ethan{method for final answer}. This structure is exemplified in Fig\ref{fig:example}. \system offers four benefits to the biological process graph generation task: first, it's a \textbf{organic reasoning approach.} \system proceeds in a way similar to how a biologist might approach the biological process term generation problem. Humans would also reason in a hierarchical, branching fashion.  
% % first identifying higher-level terms that are supported by the evidence and then proceeding to explore more specific terms. 
% Second, \system enables \textbf{contextual integration}, using well-understood biological processes as a starting point and incorporating diverse ontology information for analyzing complex gene sets. This contrasts with the simplistic approach of mapping genes to a single term, which lacks depth in problem-solving. Third, it offers high \textbf{interpretability}, as the complete graph elucidates the model's reasoning and potential errors. Fourth, \system allows for \textbf{specificity control}. It balances the abundance of higher-level terms against the detailed insights from specific terms, enabling users to navigate the trade-off between classification confidence and information content. In our analysis, we have shown that \system is able to generate significantly more relevant biological processes than the baseline models, \ethan{to write}.

% The contributions are threefold: 
% \begin{enumerate}
%     \item We propose a novel way to frame gene set analysis as a biological graph generation. The \bptree enhances the breadth and depth of gene set analysis with edge and node semantics to provide domain-specific context.
%     \item Applied \system in a sophisticated area in biology, taking gene set function as one example. 
%     \item Our analysis shows that \system can generate significantly more accurate and diverse functional terms for a gene set, and insights for future directions. 
%     \item Introduction of a novel methodology that integrates voter evaluation in the process of biological process selection and refinement, adding a layer of human-like reasoning and decision-making.
%     % \item The application of Large Language Models (LLMs) in a more structured and hierarchical approach, improving upon the current methodologies in the field.
%     % \item Demonstrating the effectiveness of the Thought Grapher through extensive evaluation, highlighting its advantages over baseline models in terms of relevancy and specificity of generated biological processes.
    
% \end{enumerate}

% In summary, our contributions are threefold: 
% \textbf{Proposing a New Task for Gene Set Analysis}: Your study introduces a novel approach to gene set analysis that encapsulates a broader diversity and greater specificity of biological processes. This represents a significant advancement over traditional methods. \textbf{Development of the ToT-Enabled Graph Generator}: You have adopted and customized the Tree-of-Thoughts (ToT) approach, leading to the creation of the ToT-Enabled Graph Generator. This tool is specifically designed for generating biological process trees, representing a key innovation in the field.

% Second, \system fosters \textbf{contextual integration}. Beginning from higher-level, well-understood biological processes and subsequently integrating information from different parts of the biological process ontology provides the model with the context to reason about more poorly understood sets of genes. By contrast, mapping the gene set to a single term without the context of neighboring or parent terms resembles the reasoning style of one who has already performed the annotation process and memorized a lookup table, rather than one who is doing novel problem solving. 
% Third, it provides high \textbf{interpretability}. The creation of a full graph allows the user to understand how the model arrived at its conclusions, and where it may have gone wrong in the reasoning process.
% Forth, it has \textbf{specificity control.} Higher-level terms in the ontology are generally more abundant than more specific terms and, as a consequence, more likely to accurately describe the gene set, but more specific terms provide more information about the gene set. As we traverse down the ontology, then, we trade confidence in our classification for information content. The optimal point in this tradeoff is subjective and varies across gene sets. This approach allows the user to inspect the full generation graph and manage the bias-variance tradeoff on a case-by-case basis, and provides automatic means of recourse if the LLM-generated answer was too specific.

% It enables exploration over coherent units of text (“thoughts”) that serve as intermediate steps toward problem-solving. 
% Several prompting schemes exist to promote complex reasoning in LLMs. Chain of thought, for example, \kyle{[finish]}. However, while chain-of-thought reasoning offers a more sophisticated approach to standard zero- or few-shot prompting, it neglects the graph-based structure of the term ontology. Rather than treat gene set analysis as a mapping problem from a set of genes to a single biological process term arbitrarily situated among thousands, a more natural approach considers where a gene set’s functions lie in the biological process graph. The biological process ontology lends itself to a reasoning scheme that similarly proceeds in a hierarchical, exploratory fashion.

% A better approach uses the Tree of Thoughts prompting framework to perform biological process term generation \kyle{cite}. We use Tree of Thoughts to build and traverse a subgraph of the biological process ontology breadth-first. In the first step, Tree of Thoughts generates three high-level candidate biological processes to describe the gene set. Among these candidates, two are chosen to proceed. In subsequent steps, Tree of Thoughts generates more specific biological processes downstream of their parent processes, along with the relation that connects the child and parent processes. At the completion of each step, the state evaluation method chooses two to keep. The state evaluator functions as a pruning mechanism for our biological process subgraph, terminating exploration among parts of the ontology that appear less salient to the gene set. At the completion of a fixed number of steps, Tree of Thoughts is asked to select a final term among the candidate terms for its final answer.



==> task.tex <==
\subsection{Task Description}
Hu et al. have explored gene set analysis as biological process generation for gene sets with GPT-4. \cite{hu2023evaluation}. However, a gene set is usually associated with a complex biological process network instead of one singular term. Generating one would lack the rich contextual information of the gene set. Therefore, we formulate the gene set analysis task as graph generation to capture the multiple aspects of a gene set, as well as, the hierarchical structure of the biological processes. 

\subsection{Problem Formulation}
Given a gene set $X = \{x_1, x_2, ..., x_n\}$, where each $x_i$ is a gene, the objective $G = F(X)$ is to design an LLM framework $F$ to generate a tree structure graph $G = (N, E)$ that represents the biological processes associated with the genes in $X$. In this graph, $N$ is the set of nodes, and $E$ is the set of edges between these nodes.

Each node $n_i \in N$ corresponds to a biological process. The tree structure of the graph implies a hierarchical relationship between these processes: the nodes at the top (root level) represent more generic biological processes and the nodes at the bottom (leaf level) represent more specific processes. The edges $E$ in the graph represent relationships or connections between different biological processes. For any two nodes $n_i, n_j \in N$, an edge $(n_i, n_j) \in E$ indicates a direct relationship between these two processes, and the relationships described in Gene Ontology are listed as follows: 
\begin{itemize}
% \setlength\itemsep{-0.5em}
\item \textbf{\texttt{is\_a}:} A is a B if biological process A is a subtype of biological process B. If A is a subtype of B, then we say A is more specific than B.

\item \textbf{\texttt{has\_part}:} A has part B if the biological process A always has part B. If A exists, then B will always exist. If A has part B, then we say B is more specific than A.

\item \textbf{\texttt{part\_of}:} A is part B if, whenever biological process A exists, it is as a part of biological process B. If A is part of B, then we say A is more specific than B.

\item \textbf{\texttt{regulates}:} A regulates B if biological process A always regulates biological process B. If A regulates B, then we say B is more specific than A.
\end{itemize}



% \subsection{Objective}
% The goal is to construct the graph $G$ from the gene set $X$ such that:
% \begin{enumerate}
%     \item $G$ is a tree, i.e., it is connected and acyclic.
%     \item The hierarchical nature of biological processes is accurately represented.
%     \item The edges $E$ meaningfully represent biological relationships between processes.
% \end{enumerate}





% Given a gene set ($x_1, x_2,...,x_n$), our goal is to generate a tree structure graph ($G$) that illustrates the given gene set’s biological processes in the form of an interconnected and organized structured network. 


% The generated graph contains nodes $n_i $ and edges$E$, $G=(N,E)$, each node $(n_1, n_2…, n_n)$ represents a biological process of the gene set (e.g., acute phase response). The nodes at the top of the tree graph are designed to be more generic and all-inclusive biological processes, and the bottom nodes represent narrow and specific concepts of the gene set. The edges denote the hierarchical relationship between nodes, described in Gene Ontolog \ethan{cite} as follows:




